Periphery-Fovea Multi-Resolution Driving Model guided by Human Attention

Inspired by human vision, we propose a new periphery-fovea multi-resolution driving model that predicts vehicle speed from dash camera videos. The peripheral vision module of the model processes the full video frames in low resolution. Its foveal vision module selects sub-regions and uses high-resolution input from those regions to improve its driving performance. We train the fovea selection module with supervision from driver gaze. We show that adding high-resolution input from predicted human driver gaze locations significantly improves the driving accuracy of the model. Our periphery-fovea multi-resolution model outperforms a uni-resolution periphery-only model that has the same amount of floating-point operations. More importantly, we demonstrate that our driving model achieves a significantly higher performance gain in pedestrian-involved critical situations than in other non-critical situations.

==> drafts.tex <==
\begin{figure}[t]
\begin{center}
\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}
\end{center}
   \caption{Example of caption.  It is set in Roman so that mathematics
   (always set in Roman: $B \sin A = A \sin B$) may be included without an
   ugly clash.}
\label{fig:long}
\label{fig:onecol}
\end{figure}


The dataset that we used, BDD-X, contains textual annotation about the driver actions and justifications. The human annotators segmented the driving videos so that during each segment the driver was doing one consistent action, \eg, going straight, slowing down and speeding up. They described the action and also the justification for that action. For example, an action annotation can be "the car is stopping" and the justification annotation can be "because a pedestrian is crossing the street". Therefore, the justifications that mention pedestrians reveal a set of various and critical driving situations where the driver had to make a reaction to a pedestrian. We tested whether our model could achieve a stronger performance gain in those pedestrian-involved critical situations than in the remaining situations which should be on average less critical.



{
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.3} 
\begin{table}[t]
	\begin{center}
	\caption{Mean testing errors of the baseline models and our driving model.}
     \label{tab:metrics}
    	\resizebox{.7\linewidth}{!}{%
    	\begin{tabular}{@{}lcccc@{}} \toprule
            Model & MAE & RMSE & Corr \\ \midrule
            No fovea & 9.6 & 14.4 & .594\\
            Random fovea & 11.2 & 15.4 & .520\\
            Central fovea & 9.4 & 13.9 & .592\\
            Human-guided fovea (top-2 fovea) & \textbf{9.1} & \textbf{13.4} & \textbf{.596}\\
            Human-guided fovea (sampled fovea) & \textbf{8.5} & \textbf{12.4} & \textbf{.626}\\ % this is sampled fovea
            High-res periphery & 6.4 & 9.8 & .723\\
            \bottomrule
        \end{tabular}}
     \end{center}\vspace{-1em}
\end{table}
}



\subsection{Fovea Location Selection}
Two independent foveae are used. In the following experiments, the fovea regionvcs can be chosen in the following selection criteria
\jinkyu{do we need to introduce all selection approaches (\ie central fovea, random fovea, human-guided fovea (top-2, sampling))? Something like}
According to our analysis, fovea regions can be chosen in the following selection criteria:
\begin{itemize}
    \item[{\bf{C.1}}] {\bf{Central Fovea Selection:}} 
    \item[{\bf{C.2}}] {\bf{Top-2 Fovea Selection:}} 
    \item[{\bf{C.3}}] {\bf{Sampled Fovea:}} 
\end{itemize}

Two independent foveae are used. The locations of the foveae are selected based on the predicted human attention map. We experimented with two methods of selecting fovea locations: top-2 and sampling. The top-2 method selects the two pixels that have the highest attention intensities in each predicted $9\times16$-pixel human attention map. The sampling method samples two fovea locations following the predicted attention probability distribution modulated by a temperature factor. This sampling method can be described by the following formula:
\begin{equation}
 p_{i} = \frac{ \exp{(\log q_{i}/T)} }{ \sum_{j}{\exp{(\log q_{j}/T)}} } 
\end{equation}
where $p_{i}$ is the probability of the i-th pixel being selected as the fovea location, $q_{i}$ is the predicted human attention probability at the i-th pixel, and $T$ is the temperature factor. A temperature factor of 1 means sampling faithfully following the predicted human attention distribution. A higher temperature factor means sampling more uniformly. A lower temperature factor means sampling more mainly from the pixel that has the highest human attention intensity.

\subsection{Foveal input extraction and foveal feature encoder}
An image patch of $240\times240$ pixels centered at each selected fovea location is cropped out from the $720\times1280$-pixel high-resolution frame images. The raw pixel values are subtracted by [123.68, 116.79, 103.939] as \cite{krizhevsky2012imagenet}. These high-resolution image patches are the foveal vision input of the model and are passed to the foveal feature encoder. The foveal convolutional feature encoder has the same structure as the peripheral feature encoder except for the kernel sizes and strides of the additional convolutional layers.


Vision-based deep autonomous driving models have shown promising results recently [refs to be added]. But their performance is still far behind humans. An important design of human vision that distinguishes it from the autonomous driving models is its multi-resolution periphery-fovea structure. Humans have high-resolution vision in the fovea that covers two degrees in visual angles. Our vision in the rest of our visual field, so called the periphery, is blurry. Our attention mechanism guides our eye movements to see the most important regions in our visual fields in high resolution. One motivation of this design is to save resources for salient regions in a redundant visual scene. Driving scenes seem to be highly redundant considering the dominating portions of uniform areas such as the sky, buildings, and roads. Inspired by the human vision, we propose a new periphery-fovea multi-resolution driving model.


High visual acuity is crucial for a vision-based autonomous driving agent. The agent depends on high visual acuity to perceive the scene at longer distances, which allows for a more advanced prediction. Many complex but subtle visual cues require high visual acuity to be processed accurately. For example, a pedestrian's gaze is a subtle cue at a visual level, but it may suggest whether the pedestrian will unexpectedly cross the street. Despite the advantages of high visual acuity, the resulting computational cost motivates the consideration of the redundancy in driving scenes. Driving scenes are commonly dominated by large portions of uniform areas such as the sky, buildings, and roads. Presumably, only small sub-regions need to be processed in high resolution. The fact that human drivers have high visual acuity only in the limited foveal region of their visual fields is a supporting evidence because they can still drive well. The fovea of the human visual system covers 2 degrees in visual angles and the remaining majority of our visual field is called the periphery and has only 0.01 - 0.2 times of the acuity of the fovea. However, humans have the attention mechanism to guide our eye movements to see the most important regions in our visual fields in high acuity. Inspired by the human vision, we propose a new periphery-fovea multi-resolution driving model to achieve both high driving performance and high efficiency.









\subsection{Peripheral-Foveal Planner}
The peripheral-foveal planner further processes the peripheral and foveal features to predict speed for the future. We experimented with two kinds of planners: combined and dual peripheral-foveal planners.

The combined peripheral-foveal planner creates foveal feature maps that have the same size as the peripheral feature maps ($9\times16$ pixels, eight semantic channels). The foveal feature maps are initialized with zeros. Each foveal image patch is encoded into a $3\times3\times8$ feature patch by the foveal feature encoder. These foveal feature patches ($\mathbf{y}_{i,j}$) are inserted into the foveal feature maps ($\mathbf{x}_{i,j}^f$) at locations corresponding to the foveal locations: 
\begin{equation}
 \mathbf{x}_{i+h,j+w}^f = \mathbf{y}_{i,j}
\end{equation}
where $h$ and $w$ are the height and width coordinates of the top-left corner of the fovea patch.

When the feature patches of two foveae would overlap, the maximum value is kept. Then the peripheral feature maps ($\mathbf{x}_{i,j}^p$) and foveal feature maps ($\mathbf{x}_{i,j}^f$) are concatenated along the semantic dimension to form the combined feature maps ($\mathbf{x}_{i,j}^c$). 
\begin{equation}
 \mathbf{x}_{i,j}^c = \Colvec{\mathbf{x}_{i,j}^p,\mathbf{x}_{i,j}^f}
\end{equation}
The combined feature maps are then processed by a ConvLSTM layer and four fully-connected layers to predict a continuous value for the vehicle speed.

The dual peripheral-foveal planner passes the peripheral features and the foveal features separately to two independent ConvLSTM layers. The outputs of the two ConvLSTM layers are then flattened and concatenated before being passed to four fully-connected layers to predict the speed. The peripheral features are $9\times16\times8$ feature maps and the foveal features are $6\times6\times8$ feature maps. To preserve the fovea location information, the positional encodings of the fovea locations are added to the foveal features.



We invented a new driving model inspired by human vision, dual-vision driving model, which has both global coarse-grained vision and local fine-grained vision. The local fine-grained vision system is guided by our previously designed human driver attention prediction model. We showed that the dual-vision driving model achieved high efficiency and better driving performance. By using the human text annotations of Berkeley DeepDrive datasets, we demonstrated that the performance gain of our model is even higher for pedestrian-involved critical driving scenarios than for other driving cases.
